Deductive Controller Synthesis for Probabilistic Hyperproperties

Probabilistic hyperproperties specify quantitative relations between the probabilities of reaching different target sets of states from different initial sets of states. This class of behavioral properties is suitable for capturing important security, privacy, and system-level requirements. We propose a new approach to solve the controller synthesis problem for Markov decision processes (MDPs) and probabilistic hyperproperties. Our specification language builds on top of the logic HyperPCTL and enhances it with structural constraints over the synthesized controllers. Our approach starts from a family of controllers represented symbolically and defined over the same copy of an MDP. We then introduce an abstraction refinement strategy that can relate multiple computation trees and that we employ to prune the search space deductively. The experimental evaluation demonstrates that the proposed approach considerably outperforms HyperProb, a state-of-the-art SMT-based model checking tool for HyperPCTL. Moreover, our approach is the first one that is able to effectively combine probabilistic hyperproperties with additional intra-controller constraints (e.g. partial observability) as well as inter-controller constraints (e.g. agreements on a common action).

==> experiments/tables.tex <==
%17-04-23: here I have prepared some tables with the latest results, so that we can do easy comparison
% TA experiment - AR
\begin{table}[H]
\centering
\begin{tabular}{ccccccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{2}{c}{Size} & \multicolumn{2}{c}{AR loop} & \multicolumn{2}{c}{HyperProb}\\
\cmidrule(rl){2-4} \cmidrule(rl){5-6}
 \textbf{Case Study} & family & MDP & time & iters & SE & SS  \\
\midrule
TA.1 (n=1) & 64   & 28   & 0.01 & 1   &  &  \\ % sat
TA.2 (n=2) & 1E6  & 76   & 0.02 & 1  &  & \\ %sat
TA.3 (n=3) & 4E12 & 148  & 0.03 & 1  &  &  \\  %sat
TA.4 (n=4) & 5E21 & 244  & 0.07 & 1 &  &     \\ %sat
\bottomrule
\end{tabular}
\captionsetup{font=small}
\caption{\textbf{TA}.}
\label{tab:TA_AR}
\end{table}

% TS experiment - AR
\begin{table}[H]
\centering
\begin{tabular}{ccccccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{2}{c}{Size} & \multicolumn{2}{c}{AR loop} & \multicolumn{2}{c}{HyperProb}\\
\cmidrule(rl){2-4} \cmidrule(rl){5-6}
 \textbf{Case Study} & family & MDP & time & iters & SE & SS  \\
\midrule
TS.0.15   & 65k & 35  & 0.01 & 1   &  &  \\ %sat
TS.10.20  & 2E6 & 45  & 0.01 & 1  &  & \\ %sat
TS.8.15   & 65k & 35  & 0.01 & 1  &  &  \\  %sat
TS.0.1    & 4   &  7  & 0.01 & 1 &  &     \\%sat
TS.4.8    & 512 &  21  & 0.01 & 1 &  &     \\%sat
\bottomrule
\end{tabular}
\captionsetup{font=small}
\caption{\textbf{TS}.}
\label{tab:TS_AR}
\end{table}

% the one in which we are slower.
\subsection{Probabilistic Conformance}
Probabilistic Conformance (\textbf{PC}) is a synthesis benchmark packaged with HyperProb. Consider the well-known Knuth-Yao algorithm for simulating a fair 6-sided die by repeatedly tossing a fair coin. The benchmark assumes no knowledge of the probabilities of each outcome, but compares an MDP model with the actual 6-sided die represented by a DTMC, and uses some hyperproperties to express the requirement that they should induce the same distribution over the outcomes.

% PC experiment - AR
\begin{table}[H]
\centering
\begin{tabular}{ccccccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{2}{c}{Size} & \multicolumn{2}{c}{AR loop} & \multicolumn{2}{c}{HyperProb}\\
\cmidrule(rl){2-4} \cmidrule(rl){5-6}
 \textbf{Case Study} & family & MDP & time & iters & SE & SS  \\
\midrule
PC.0  & 156   & 20 & 1.17        & 152   &  &  \\ % sat
PC.1  & 6084  & 20 & 36.17       & 5566  &  & \\ %sat
PC.2  & 474k  & 20 & 146.39      & 20k   &  &  \\  %sat 
PC.3  & 4E7   & 20 & 2455.93     & 320k  &  &     \\ %sat
PC.4  & 3E9   & 20 & \texttt{TO} &       &  &     \\ %sat
PC.5  & 2E10  & 20 & \texttt{TO} &       &  &     \\ %sat
PC.6  & 2E13  & 20 & \texttt{TO} &       &  &     \\ %sat
\bottomrule
\end{tabular}
\captionsetup{font=small}
\caption{\textbf{PC}.}
\label{tab:PC_AR}
\end{table}







==> sections/counterexamples.tex <==
% CEGIS ---------------------------------
\subsection{Counterexample-guided synthesis}
\todo{This whole section can go to appendix. In the main text, we can just intuitively describe the key conceptual difference between CE and CE-based synthesis for standard PCTL and hyperproperties. We would also say that the current implementation of CE-based synthesis have a significant computational overhead  and thus it does not improve the AR algorithm. What do you think?}


A m-MC $\mathcal{M}^{\sigma_r}$ induced by a controller $\sigma_r$ that violates a specification $\varphi$ (i.e. $\mathcal{M}^{\sigma_r} \nvDash \varphi$)
provides a crucial source of information for searching for a satisfying solution. Following the notion of \emph{critical subsystems} \cite{QuatmannJDWAKB15,AbrahamBDJKW14,HanKD09}, we define \emph{counterexamples} (CEs) for probabilistic hyperproperties. We then extend the approach of \cite{Andriushchenko021} and use the CEs to compute  efficiently from $\mathcal{M}^{\sigma_r}$ a set of realisations $\mathcal{R}' \subseteq \mathcal{R}^{\sigma_{K}}$ that also violate $\varphi$ and thus can be safely prunned. 
 
%\todo{There has to be an intuitive explanation what is CE for hyperproperites -- emphasize that the difference to the regular CEs. Also, it has to be explained that we consider only 2 computational trees} 

%As we focus only on the set of 2-hyperproperties, the generation of a CE has to compare two computation trees, the ones determined by the two probability expressions in the inequality (recall that functions of probability expressions allow to generalize to n-hyperproperties). Given the two trees and the $\leq$ inequality relation, a Counterexample is the union of two subtrees such that, for every possible extension of them, the inequality does not holds. This means idetifying two subtrees with two critical probability masses. 


Hyperproperties reason about multiple computation trees and thus the CE needs to include multiple sub-trees  witnessing the violation of the hyperproperty. As before, we restrict ourselves to the class of 2-hyperproperties. Consider a property $\varphi = \llinstfullsprob{1}{1}{T_1} \leq \llinstfullsprob{2}{2}{T_2}$ that is violated by the induced m-MC $\mathcal{M}^{\sigma_r}$. Recall that the state-space of $\mathcal{M}^{\sigma_r}$ is given by $\bigcup_{i=1}^m S_i$. Intuitively, for $\varphi$, the CE is given by a pair of sets $C_1\subseteq S_1$ and $C_2\subseteq  S_2$ inducing in $\mathcal{M}^{\sigma_r}$ two sub-trees  rooted in $s_1$ and $s_2$, respectively, having a critical probability mass ensuring that the probability of reaching $T_1$ from $s_1$ is \textbf{larger} than the probability of reaching $T_2$ from~$s_2$. 

For the LHS of the inequality in $\varphi$, we rely on the usual notion of CEs for \emph{safety} properties, which identifies as a CE a sub-tree with critical probabability mass that exceeds the safety threshold. For the RHS, we make use of the definition of CEs for \emph{liveness} properties, where a CE is specified by resorting to computing a safety CE for the probability of \textbf{not} reaching the target. That is, a CE is a sub-tree such that the probability of reaching a bottom SCC without any state in the target exceeds one minus the original liveness threshold. With respect to an hyperproperty, such two safety and liveness thresholds are not fixed by the formula, as in the case of the standard CEs for PCTL, but are computed dynamically, and are represented respectively by the probability obtained by the other sub-tree of the pair. The two probability masses and the two sub-trees are hence critical \emph{not per se}, but in relation with each other.

% \begin{definition}[Counterexample] \label{def:Ce}
% Let $\mathcal{D} = \mathcal{M}^{\sigma} = (\mathcal{S}, \mathcal{I}, Act, \mathfrak{p}^{\sigma})$ be an induced MC on the m-replication $\mathcal{M}$ of MDP $M := (S, I, Act, \lltrans)$. Assume $s_{\bot}, s_{\top} \notin S$. The sub-MC of $\mathcal{D}$ induced by $C \subseteq \mathcal{S}$ is the MC $\mathcal{D}{\downarrow}C = (\mathcal{S} \cup \{s_{\bot}, s_{\top}\}, \mathcal{I}, (\mathfrak{p}^{\sigma})' ) $, where the transition probability function $(\mathfrak{p}^{\sigma})'$ is defined by:
%   \begin{equation*}
%     (\mathfrak{p}^{\sigma})' (s) =
%     \begin{cases*}
%       \mathfrak{p}^{\sigma(s)} & if $s \in C$ \\
%       [s_{\bot} \mapsto 1]  & if $s \in S_{1} \backslash C$ \\
%       [s_{\top} \mapsto 1]  & if $s \in S_{2} \backslash C$ \\
%     \end{cases*}
%     \end{equation*}

% The set $C$ and the sub-MC $\mathcal{D}{\downarrow}C$ are called a \textup{counterexample} (CE) for the hyperproperty $\llinstfullsprob{1}{1}{T_1} \leq \llinstfullsprob{1}{2}{T_2}$ on MC $\mathcal{D}$, if $\mathcal{D}{\downarrow}C \nvDash \llmreplicatedfullsprob{1}{1}{(T_1 \cap (C \cup {s_{1,1}}))} \leq 1 - \llmreplicatedfullsprob{1}{2}{(B \cap (C \cup s_{1,2}))}$, where $B$ is the set of states in $\mathcal{D}$ that do not have a path to $T_2$.
% \end{definition}

% $B$ can be computed with standard methods \cite{0020348}.

%\descr{2) Define the family-aware CE (using the bounds as the hybrid approach).}


Following the results of \cite{Andriushchenko021}, we use a refined version of the CEs. Instead of requiring that
\emph{every possible extension} of the CE violates the hyperproperty, we consider only \emph{extensions that corresponds to a family member}. As shown in \cite{Andriushchenko021}, such family-aware CEs are typically smaller which is crucial for having an effective pruning strategy. We now lift the notation of family-aware CEs to 2-hyperproperties. Let us assume that for the given family of controllers $\sigma_K$, we have for each state $s\in S$ an upper bound $ub^{\sigma_K}(s,T_1)$ on the probability to reach $T_1$ and a lower bound $lb^{\sigma_K}(s,T_2)$ on the probability to reach $T_2$, i.e. $\forall \sigma \in \sigma_K, s\in S: ub^{\sigma_K}(s,T_1) \geq \reach{\sigma,s}{T_1} \wedge  lb^{\sigma_K}(s,T_1)\leq \reach{\sigma,s}{T_2}$. Note that, We can effectively obtain these bounds by model-checking the replicated MDP $\rmdp$.

%\textcolor{red}{TBD: Formal definition of family-aware CE for 2-hyperproperties, explaining how CE can be used in pruning -- conflicts}

\begin{definition}[Family-aware counterexample]
Consider a family of controllers $\sigma_K$ over m-replication $\rmdp $ and a controller $\sigma_r \in \sigma_K$ inducing a m-MC $\rmdp^{\sigma_r} = \bigcup_i^m M_i^{r \circ \sigma_{K}}$, where MC $M_i^{r \circ \sigma_{K}} = (S_i,\mpm_i)$, that violates a 2-hyperproperty $\varphi = \llinstfullsprob{1}{1}{T_1} \leq \llinstfullsprob{2}{2}{T_2}$. Let $ub^{\sigma_K}(s,T_1)$ and $lb^{\sigma_K}(s,T_2)$ be the upper and lower probability bounds for reaching $T_1$ and $T_2$ in $\sigma_K$, respectively. A pair ($C_1 \subseteq S_1,  C_2 \subseteq S_2$) is a counterexample with respect to $\sigma_r$ and $\varphi$ in the family $\sigma_K$ if 
$$\reach{M_1^{r \circ \sigma_{K}}\downarrow C_1,s_1}{T_2} > \reach{M_2^{r \circ \sigma_{K}}\downarrow C_2,s_2}{T_2}, $$
where $M_i^{r \circ \sigma_{K}}\downarrow C_i$ for $i\in \{1,2\}$ are two MCs defined as follows. 
$M_i^{r \circ \sigma_{K}}\downarrow C_i = (S_i \cup \{s_{\bot}, s_{\top}\}, \mpm_{C_i})$ with 

\begin{equation*}
    \mpm_{C_i} (s)
     \begin{cases*}
        \mpm_1(s) & if $s \in C_i$ \\
           [s_{\top} \mapsto \gamma_i(s,T_1), s_{\bot} \mapsto (1 - \gamma_i(s,T_1)]  & if $s \in S_1 \backslash C_1$ \\
           [s \mapsto 1]  & if $s \in \{ s_{\top}, s_{\bot}\}$ \\
    \end{cases*}
\end{equation*}
with $\gamma_1(s,T_1) =  ub^{\sigma_K}(s,T_1)$ and $\gamma_2(s,T_2) =  lb^{\sigma_K}(s,T_2)$.
\end{definition}


From a CE $C=(C_1,C_2)$ with respect to $\sigma_r$ and $\varphi$ in $\sigma_K$, we can easily compute the set of realisations $\mathcal{R}' \subseteq \mathcal{R}^{\sigma_{K}}$ violating $\varphi$. Let $K_C = \bigcup_{s \in C_1 \cup C_2} \sigma_{K}(s)$ be a set of relevant parameters (so-called \emph{conflict}) for the CE $C$. Then $\mathcal{R}' = \{r\in \mathcal{R}^{\sigma_{K}} \mid \forall k \in K_C : $ $r(k) = r'(k)\}$. 
The number relevant parameters $K_C$ is crucial.
Small conflicts potentially lead to larger subfamilies $\mathcal{R}'$.
It is thus important that the CEs contain as few parameterized transitions as possible. 
The size of a CE in terms of the number of states is not of interest. 
Furthermore, the overhead of providing CEs should be bounded from below by the payoff: Finding a large generalization may take some time, but small generalizations should be returned quickly.
Existing off-the-shelf CE-generation procedures \cite{DehnertJWAK14,abs-1305-5055} do not feature the awareness of the family, and do not target probabilistic hyperproperties. Therefore, we extend the approach from ~\cite{Andriushchenko021}, that greedily generated family-aware CEs minimising the 
 the number of relevant parameters, to work with hyperproperties. \todo{Add a short informal description of the greedy algorithm}



% Instead of extending them, we devise an oracle with the following features:
% \begin{itemize}
%     \item it is \emph{greedy}: the generation of minimal counterexamples is a NP-hard problem\cite{FunkeJB20}. While it takes time to compute them, they do not give any guarantee about the optimality of the induced conflict. We resort to a greedy approach that produces rapidly good but non optimal CEs.
%     \item it is \emph{aware of the presence of parameters}, and how states are mapped to parameters. Instead of trying to minimizing the number of states, it tries to minizing the number of relevant parameters in the CE.
%     \item it generates \emph{family-aware CEs}, as described above, by using an abstraction over the family $\sigma_{K}$.
% \end{itemize}

% In practice, the oracle enforces an iterative and incremental state exploration approach of $\mathcal{D}_{r}$. Initially, $C^{(0)} = \varnothing$, i.e., all states are rerouted, and the set of relevant parameters $K^{(0)} = \varnothing$. If this is already a CE, the entire family is discarded, and the algorithm terminates. Otherwise, consider iteration $i$. The oracle expands all states that are reachable from $s_{1,1}$ or $s_{1,2}$ via states that are mapped to a parameter $k \in K^{(i)}$. Such states constitute $C^{(i)}$. Assume $\varphi'$ is the updated hyperproperty, and that it finds out that $\mathcal{D}_{r}{\downarrow}C^{(i)}[\mathbf{\gamma}] \vDash \varphi'$. The oracle then examines $H^{(i)}$, the state exploration ``horizon''. $H^{(i)}$ consists of those states that are reachable from $s_{1,1}$ or $s_{1,2}$ but have not been expanded yet, which means that they are mapped to an irrelevant parameter. Let $K_{H^{(i)}}$ be the parameters mapped from at least one state in $H^{(i)}$. The oracle, \emph{greedily}, chooses the member $k'$ of $K_{H(i)}$ that is mapped from the highest amount of states in $H^{(i)}$, and adds it to the conflict. It then moves to the subsequent iteration, where we have $K^{(i+1)} = K^{(i)} \cup k'$, and hence $C^{(i+1)} \supset C^{(i)}$. Expanding more states cannot decrease the reachability probability from $s_{1,1}$ as $lb^{\mathcal{R}}(\lleven T_1)$ is a valid lower bound, and cannot increase the reachability probability from $s_{1,2}$ as $ub^{\mathcal{R}}(\lleven T_2)$ is a valid upper bound. This gradual expansion strategy is guaranteed to terminate as $\mathcal{D} \vDash \varphi \iff \mathcal{D}{\downarrow}(S_1 \cup S_2)[\gamma] \vDash \varphi'$ (as only states in $S_1 \cup S_2$ are relevant for the computation of reachability probabilities), and our initial assumption is $\mathcal{D} \nvDash \varphi$.


\subsection*{Q3: Conterexamples - Integrated Method} 
% ProbNI - HYBRID (all unsat) [comparison with Hybrid]
\begin{table}[H]
\centering
\begin{tabular}{c  c  cc  ccc}
\toprule
\multirow{2}{*}{Controller(s)} & \multirow{2}{*}{Memory} & \multicolumn{2}{c}{AR loop} & \multicolumn{3}{c}{CEs-integrated}\\
\cmidrule(rl){3-4} \cmidrule(rl){5-7}
 & & time & iters & time & AR iters & CEs \\
\midrule
\multirow{2}{*}{two} & no   & 0.09 & 7 & 0.08 & 1 & 4\\ 
                     & yes(1-bit) & 481.33 & 16k & 827.19 & 13k & 26k \\
\bottomrule
\end{tabular}
\captionsetup{font=small}
\caption{\textbf{Probabilistic Noninterference} - comparison between the pure AR method and the integration of CEs.}
\label{tab:ProbNI:Hybrid}
\end{table}

% SD HYbrid
\begin{table}[H]
\centering
\begin{tabular}{c cc  ccc}
\toprule
\multirow{2}{*}{ \textbf{Maze}} & \multicolumn{2}{c}{AR loop} & \multicolumn{3}{c}{CEs-integrated}\\
\cmidrule(rl){2-3} \cmidrule(rl){4-6}
  & time & iters & time & AR iters & CEs \\
\midrule
smaller        & 1.11        & 1.5k & 2.46 & 1.6k & 555  \\
larger-sat     & 177.27(8\%) & 171k & 369.38(16\%) &  163k & 45k  \\
larger-unsat   & 443.25      & 442k & 872.56  & 388k & 107k \\
larger-sat-2   & 0.11(10\%)  & 119  & 0.25(10\%) & 116 & 25  \\ 
splash         & 1731.33     & 1E6  & 2547.84 & 1E6 & 299k    \\ 
splash-easy    & 0.04(10\%)  & 63   & 0.1(10\%) & 63 & 12  \\
train          & 7.27        & 8.7k & 15.36 & 7.8k & 1.8k      \\
\bottomrule
\end{tabular}
\captionsetup{font=small}
\caption{\textbf{SD} on different Mazes - comparison between the pure AR method and the integration of CEs.}
\label{tab:SD_Hybrid}
\end{table}
